Characterizing and Mitigating the Impact of Telluric Absorption in Precise Radial Velocities

Precise radial velocity (PRV) surveys are important for the search of Earth analogs around nearby bright stars. Such planets induce a small stellar reflex motion with RV amplitude of $\sim$10 cm/s. Detecting such a small RV signal poses important challenges to instrumentation, data analysis, and the precision of astrophysical models to mitigate stellar jitter. In this work, we investigate an important component in the PRV error budget - the spectral contamination from the Earth's atmosphere (tellurics). We characterize the effects of telluric absorption on the RV precision and quantify its contribution to the RV budget over time and across a wavelength range of 350 nm - 2.5$\mu$m. We investigate the effectiveness in mitigating tellurics using simulated spectra of a solar twin star with telluric contamination over a year's worth of observations, and we extracted the RVs using two commonly adopted algorithms: dividing out a telluric model before performing cross-correlation or Forward Modeling the observed spectrum incorporating a telluric model. We assume various degrees of cleanness in removing the tellurics, including mimicking the lack of accurate knowledge of the telluric lines by using a mismatched line profile to model the "observed" tellurics. We conclude that the RV errors caused by telluric absorption can be suppressed to close to or even below the photon-limited precision in the optical region, especially in the blue, around 1-10 cm/s. At red through near-infrared wavelengths, however, the residuals of tellurics can induce an RV error on the m/s level even under the most favorable assumptions for telluric removal, leading to significant systematic noise in the RV time series and periodograms. If the red-optical or near-infrared becomes critical in the mitigation of stellar activity, systematic errors from tellurics can be eliminated with a space mission such as EarthFinder.

==> recycle.tex <==
% Recycle bin for texts

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Old Methodology Texts
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

(water, ch4, co2, n2o, o2, o3) The TAPAS spectras *generates* will be downloaded in the form of  .ipac files, with 6 *objects* in each of the 12 folders,\textbf{ one for each month.} In order to be able to use the TAPAS files as needed with more efficiency, it becomes worthwhile to convert each of the files to .npz files. This can increase the speed with which the next step can be done, which is plotting these .npz files, and saving the plots as a .png file. This can again be done with a simple loop, and will move far faster than if done with .ipac files.


We simulated observed spectra over the course of one year (365 nights) on the Sun using the Kurucz solar spectrum generated by ATLAS9 \citep{kurucz2005}. We added telluric absorption in each simulated spectrum using synthetic telluric spectra generated by TAPAS \citep{tapas}. We generated 12 sets of synthetic telluric spectra using TAPAS at midnight on the middle day of each month in 2017, using the atmospheric profile models for the Kitt Peak National Observatories as provided by TAPAS through the ETHER service. We generated the spectra for six molecules separately (water, methane, CO2, N2O, O2, O3), without additional line broadening and at the highest resolution and sampling possible, without Rayleigh scattering, and at airmass = 1.0.
 
For the simulated spectrum of each night, we add the telluric spectrum in the following way: \begin{enumerate}

\item We randomly draw a number for airmass from a Gaussian distribution centered at 1.25 with width 0.2, which resembles the airmass distribution of the RV standard star HD 10700 (tau Ceti) as observed by Keck/HIRES. Then, we choose the starting set of six telluric spectra (one for each molecule) from the corresponding month. We scale the spectra of the relatively stable constituents of the atmosphere (methane, CO2, N2O, O2, O3, i.e. everything but water) by the airmass through a simple power law scaling (fscaled = f airmass). We have verified that this simple power law works well even for deep and saturated lines by comparing the scaled spectra with the ones generated by TAPAS at airmass 
\item We randomly draw a value for the amount of precipitable water vapor (PWV; units mm) from a Gaussian distribution centered at 5.0 mm with width 2.0 mm, which resembles the PWV distribution of Kitt Peak in 2017 as recorded by Suominet (https://www.suominet.ucar.edu/). We apply an upper limit of 10 mm because with PWV > 10 mm the weather condition is typically not suitable for astronomical observations. We then scale the input TAPAS water spectrum (from a night with very low PWV, 1.8 mm) according to the airmass and PWV values drawn to get the correct line depths.
\item We determine the barycentric velocity correction (BC; the relative velocity between the observatory and the star due to Earth’s motion around the solar system barycenter) of the “observed star” for that night following

\begin{center} BC = (date / 365 2-/2)30 km/s, CHECKCHECKCHECK \end{center}

which roughly matches with the BC values throughout a year for tau Ceti as observed at Keck. Then we shift the telluric spectra according to the BC value to offset the telluric spectra from the stellar spectrum in RV space to mimic the Earth’s motion.
\item  We then multiply the shifted telluric spectra with the stellar spectrum. We chose to shift the telluric spectra instead of the stellar spectrum (the synthetic solar spectrum) because the telluric spectra have a higher fidelity, and by minimizing manipulating the stellar spectrum we avoid adding extra numerical errors that would affect the extracted RVs. This means that the true RVs for all spectra would be 0 m/s.
\item We then convolved the spectrum to a spectral resolution of R=120,000, which is representative of the spectral resolution of the next-generation ground-based PRV instruments. We did not bin the spectrum further down to mimic the CCD pixels but chose to preserve the original binning of the Kurucz solar spectrum to avoid further numerical errors. As a result, the “pixel size” in our simulated spectra is about 0.0007-0.005 nm, a factor of three smaller than the typical CCDs used for PRV instruments today. We chose not to add photon noise or blaze function in our simulated spectra to avoid adding more RV errors in order to isolate the effects of tellurics.
\end{enumerate}

Next, we extracted RVs from the simulated spectra with three different methods:the effects of tellurics are extracted via computation of a cross-correlation function (CCF) method following \citet{baranne1996}. The CCF is performed between the simulated observed spectra and a “template” spectrum that is exactly the same as the input stellar spectrum convolved in the exact same way to R=120,000. This means that we assume a perfectly known spectral point spread function (PSF) and wavelength solution, which are not unrealistic for the ultra-stabilized next-generation spectrographs calibrated by laser frequency combs. The assumption of a perfect stellar template, however, is not realistic, but we chose to do so to isolate the effects of tellurics.

\begin{enumerate}

\item Division: RVs are extracted via a CCF but before the CCF is computed, a telluric spectrum is removed via mathematical division. The telluric spectrum being divided out is exactly the same one as used for generating the simulated spectrum for each night and convolved to R=120,000 in the same fashion. This division then the CCF method is the most commonly used method to mitigate the effects of tellurics in PRVs for stabilized spectrographs such as HARPS and CARMENES.

\item Modeling: RVs are extracted via the forward modeling method similar to \citet{butler1996}. This methods builds a model using the stellar template and the synthetic telluric spectra, with the Doppler shift or RV, a linear correction on the continuum, and the column density or power-law scaling of the telluric molecular lines as free parameters, to fit the observed spectrum via least-chi square minimization. Again we assumed perfectly known wavelength solution and spectral PSF. Telluric fitting is not turned on for a spectral chunk unless the absorbed flux by a certain molecule exceeds 0.1\% in our input model telluric spectrum, following Wang et al. (2018). In the results presented below for the Modeling method, instead of using the telluric spectra exactly the same as the ones synthesized into the observed spectrum just like in the Division method, we used a different set of telluric spectra with the wrong line profiles as the model input to mimic our lack of knowledge of the atmospheric conditions and molecular line profiles. This set of telluric spectra with the mismatched line profiles were generated by TAPAS using atmospheric conditions of Mauna Kea (instead of Kitt Peak) at the midnight of  January 15, 2017. Figure 3.2.1 illustrates this mismatch of line profile.
\end{enumerate}

When extracting RVs, we divided each spectrum into 230 chunks, from 0.3 nm at 350 nm to about 20 nm at 2.5 μm, growing linearly as the wavelength. The change of chunk size is to mimic the length of a typical spectral order and also to compensate for the decrease of Doppler content in the solar spectrum towards the NIR.
To validate our CCF algorithms, we performed CCF on a telluric-free solar spectrum and confirmed that it returns the correct RV (0 m/s) for all spectral chunks. We also validated our forward modeling algorithm by using the exact same telluric spectra as the modeling input, and the modeling code returned 0 m/s for all spectral chunks in all 365 nights of spectra. This is another reason why we introduced the line profile mismatch for the Modeling method.

OTHER OLD TEXTS.
In order to simulate an observed spectra with some accuracy, several steps had to be taken to ensure a realistic 'observation', so to speak. In order to maintain realism, the program had to accurately account for barycentric correction, precipitable water vapor, and airmass, if given a date in the year. This was done in a threefold process:
\begin{enumerate} 
\item For the barycentric correction, the equation $\sin{(\frac{date}{365.15\cdot 2\pi}-\frac{\pi}{2.0})}\cdot(3\times10^4)$ accurately accounted for the relative velocities of *all moving parts*TO BE CHANGED. 
\item For the precipitable water vapor, or PWV, a random number generator was used *MORE HERE ON SPECIFICATIONS*, with the caveat that  if the PWV was greater than 10 UNIT?, it was reset to be equal to 10 UNIT?, and a PWV less than 1.8 UNIT?, it was set to be equal to 1.8 UNIT?. 
\item This same concept stated above was applied to the airmass, however, there were two changes. Firstly, *MORE ON SPECIFICATIONS HERE*. Secondly, if the airmass was greater than 2.0 UNIT, it was set to be equal to 2.0 UNIT, and if less than 1.0 UNIT, it was set to be equal to 1.0 UNIT.
\end{enumerate}
The next step is to be able to feed a PWV and date into the program, and have it return the appropriate TAPAS file. *MORE HERE*
After this, the telluric spectra are blended, shifted, and convolved. 
%% The "ht!" tells LaTeX to put the figure "here" first, at the "top" next
%% and to override the normal way of calculating a float position


%\newpage

BREAKBREAKBREAKBREAKBREAKBREAKBREAKBREAKBREAKBREAK

FROM REPORT
We simulate observed spectra over the course of one year (365 nights) on the Sun using the Kurucz solar spectrum generated by ATLAS9 \citep{kurucz2005}. We add telluric absorption in each simulated spectrum using synthetic telluric spectra generated by TAPAS \citep{tapas}. Overall, our simulation aims to reproduce an ensemble of realistic spectra of a Sun-like star through the Earth’s atmosphere throughout a year, and we then extract RVs from these spectra using different telluric mitigation methods and compare their effectiveness. We briefly describe our methodology below.

For each night, we randomly assign an airmass for the observation and scale the telluric absorption to the appropriate depths. The distribution of the airmass resembles a typical star observed frequently throughout a year. In addition, we randomly draw a value for the amount of precipitable water vapor (PWV; unit is mm) and scale the water lines accordingly. The PWV values are drawn from a distribution that resembles the PWV values of astronomical nights at Kitt Peak in 2017 as recorded by Suominet (https://www.suominet.ucar.edu/). The telluric spectrum and the stellar spectrum are offset in wavelength space before being combined together according to the barycentric velocity correction (BC, the relative velocity between the observatory and the star due to Earth’s motion around the solar system barycenter) of the star, for which we used the approximation of a sine curve over a year with a semi-amplitude of 30 km/s (e.g. for stars near the celestial equator). 

We then convolve the spectrum to a spectral resolution of R=120,000, which is representative of the spectral resolution of the next-generation ground-based PRV instruments. We do not bin the spectrum further down to mimic the CCD pixels but chose to preserve the original binning of the Kurucz solar spectrum to avoid further numerical errors. As a result, the “pixel size” in our simulated spectra is about 0.0007-0.005 nm, a factor of three smaller than the typical CCDs used for PRV instruments today. We choose not to add photon noise or blaze functions in our simulated spectra to avoid adding more RV errors in order to isolate the effects of tellurics.
Next, we extract RVs from the simulated spectra with three different methods:
\begin{enumerate}
\item  No correction: RVs are extracted via computation of a cross-correlation function (CCF) method following \citet{baranne1996}. We assume a perfectly known spectral point spread function (PSF), and wavelength solution, which are not unrealistic for the ultra-stabilized next-generation spectrographs calibrated by laser frequency combs. We also use a perfectly known stellar template to perform the CCF, which is unrealistic but allows us to isolate the effects of tellurics.
\item  Division: RVs are extracted via a CCF but before the CCF is computed, a telluric spectrum is removed via mathematical division. The telluric spectrum being divided out is exactly the same one as used for generating the simulated spectrum for each night and convolved to R=120,000 in the same fashion. This approach is the most commonly used method to mitigate the effects of tellurics in PRVs for stabilized spectrographs such as HARPS and CARMENES.
\item Modeling: RVs are extracted via the forward modeling method similar to \citet{butler1996}. This method builds a model using the stellar template and the synthetic telluric spectra, with the Doppler shift or RV, a linear correction on the continuum, and the column density or power-law scaling of the telluric molecular lines as free parameters, to fit the observed spectrum via χ2 minimization. We again assume a perfectly known wavelength solution and spectral PSF. Telluric fitting is not turned on for a spectral chunk unless the absorbed flux by a certain molecule exceeds 0.1\% in our input model telluric spectrum, following \citet{thesis} RVs are extracted via the forward modeling method similar to \citet{butler1996}. This method builds a model using the stellar template and the synthetic telluric spectra, with the Doppler shift or RV, a linear correction on the continuum, and the column density or power-law scaling of the telluric molecular lines as free parameters, to fit the observed spectrum via χ2 minimization. We again assume a perfectly known wavelength solution and spectral PSF. Telluric fitting is not turned on for a spectral chunk unless the absorbed flux by a certain molecule exceeds 0.1tes this mismatch of line profile.
\end{enumerate}



When extracting RVs, we divide each spectrum into 230 chunks, from 0.3 nm at 350 nm to ~20 nm at 2.5 $\mu$m, with chunk size growing linearly as the wavelength. The change of chunk size is to mimic the length of a typical spectral order and also to compensate for the decrease of Doppler content towards the NIR.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
